Leaked-Web: Accurate and Efficient Machine Learning-Based Website Fingerprinting Attack through Hardware Performance Counters

Users' website browsing history contains sensitive information, like health conditions, political interests, financial situations, etc. Some recent studies have demonstrated the possibility of inferring website fingerprints based on important usage information such as traffic, cache usage, memory usage, CPU activity, power consumption, and hardware performance counters information. However, existing website fingerprinting attacks demand a high sampling rate which causes high performance overheads and large network traffic, and/or they require launching an additional malicious website by the user, which is not guaranteed. As a result, such drawbacks make the existing attacks more noticeable to users and corresponding fingerprinting detection mechanisms. In response, in this work, we propose Leaked-Web, a novel accurate and efficient machine learning-based website fingerprinting attack through processor's Hardware Performance Counters (HPCs). Leaked-Web efficiently collects hardware performance counters in users' computer systems at a significantly low granularity monitoring rate and sends the samples to the remote attack's server for further classification. Leaked-Web examines the web browsers' microarchitectural features using various advanced machine learning algorithms ranging from classical, boosting, deep learning, and time-series models. Our experimental results indicate that Leaked-Web based on a LogitBoost ML classifier using only the top 4 HPC features achieves 91% classification accuracy outperforming the state-of-the-art attacks by nearly 5%. Furthermore, our proposed attack obtains a negligible performance overhead (only <1%), around 12% lower than the existing hardware-assisted website fingerprinting attacks.

==> sections/date-review.tex <==
============================================================================
                            REVIEWER #1
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                           Overall Value: -3

Summary of ideas
---------------------------------------------------------------------------
The paper proposes to use hardware performance counters for fingerprinting websites that users visit.  The approach has a low performance impact and high accuracy.
---------------------------------------------------------------------------


Strong points
---------------------------------------------------------------------------
* Low performance impact
---------------------------------------------------------------------------


Weak points
---------------------------------------------------------------------------
* Unrealistic (and not explicitly specified) threat model
* Unfair comparison to past work
* Incomplete description of some experiments
* The paper could use a pass by a professional editor
---------------------------------------------------------------------------


Other comments
---------------------------------------------------------------------------
I read the paper with interest and, while I appreciate the work that has gone into the paper, I am afraid that I am unable to recommend acceptance to the program.

The main limitation of the paper is that the threat model is not clear.  The paper never explicitly states the threat model, and the implied model requires the attacker to be able to run performance monitoring on the victim.  For this, the paper requires setting the perf_event_paranoid to a non-default, insecure value.  This is unlikely to be a realistic scenario.  

The paper does not explain how Challenge 2 is overcome.  For Chrome with strict site isolation, this may be done by monitoring only a single process (but the attacker needs to know which process to monitor).  For Firefox, the paper needs to demonstrate that the technique works even when a large number of tabs and windows are open.

The paper only experiments with 30 sensitive sites.  This is much lower than other works it compares against.  The number of sensitive sites has a significant impact on accuracy, and the paper cannot claim a better accuracy when using a lower number of sites.

The paper does not fully describe the open-world settings.  It is not clear how many traces of the non-sensitive sites are used for the training and the attack phases.  The paper also fails to explain how it handles the unbalanced dataset in this settings.  Moreover, the paper claims that the open-world setting is a binary classification problem.  This does not match past work, where the classifier needs to identify the site if the site is sensitive.

**Minor comments**  
Introduction: A "web browser fingerprint" usually refers to a fingerprint that identify the web browser to the web server.  The paper deals with website finerprints.

Section II-B: I have no idea what Adaboost is.

Section II-C: Tor is not a network-based anomaly detection.

Section III-B: 1^6 and 1^0 are both equal to 1.

Section IV-B claims that the accuracy in open-world decreases by 2-3%, but Figure 8 shows that it increases.

There is a large number of language issues in the paper.  Examples include "to to" in the abstract, "and etc." in the introduction, and more.  I suggest getting a professional editor to review the paper.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                           Overall Value: -1

Summary of ideas
---------------------------------------------------------------------------
This paper discusses Hardware Performance Counter (HPC) based fingerprinting for webpages. By assuming access to the users' processor through native code execution (e.g., via a malicious browser extension), the impact of different webpages on the microarchitectural state can be monitored and classified. This gives rise to the Leaked-Web attack, which first learns the features of existing webpages, after which it can classify them during runtime. The main contribution of this work is that the overhead of the malicious code is reduced by decreasing the sampling rate of the HPCs, without any loss (even an increase) in classification accuracy.
---------------------------------------------------------------------------


Strong points
---------------------------------------------------------------------------
The paper is well written and easy to read. The topic is interesting and the results are good: 91% classification accuracy with only 1% overhead for a user.
---------------------------------------------------------------------------


Weak points
---------------------------------------------------------------------------
The main weakness is that contribution is very incremental: the reference [7] should be given much more credit than being called a "similar previous work". Essentially everything this paper proposes was already achieved in [7], except that the current work tweaks the setup by 1) decreasing the sampling rate and 2) using alternative ML algorithms. Although it is nice to show that the results do not significantly decrease at lower sampling rates, this is fairly incremental. In particular, giving this attack its own name seems a bit much being so derivative from [7].

I am also a little confused about the various claims about ease of execution. It is mentioned at several points that no malicious web page or local malware needs to be set up, which is an advantage compared to existing work [11, 22, 23]. But there seems to be little elaboration on what *is* required to run the attack. How does one actually get access to HPCs on a users' device? It appears that a malicious browser extension is required, but this is not clarified anywhere. In similar fashion, how is the training data set obtained? Surely it is not so straightforward to get on the users' device, does it suffice to create this locally on the same platform?
---------------------------------------------------------------------------


Other comments
---------------------------------------------------------------------------
* p1: "to to cope"
* p1: "behaviour" later spelled as "behavior"
* p1: "Conduct businesses" -> "conduct business"
* p2: "another drawbacks" -> "another drawback"
* p2: [7] looks at Chrome and Tor, not Firefox
* p3: The Tor projection is described as "anomaly detection", but its purpose is of course more to avoid than to detect
* p5: "train various"
* p6: In Fig. 8 the y-axis label has a "9" instead of "("
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                           Overall Value: -1

Summary of ideas
---------------------------------------------------------------------------
The paper deals with hardware performance counters for website fingerprinting.
Experiments are performed on an intel i5, with 4 cores running Ubuntu 20.04 using Chrome and Firefox.
---------------------------------------------------------------------------


Strong points
---------------------------------------------------------------------------
- important research topic
- low-performance overhead
- high success rate (in the considered setup)
- straightforward to follow
- consideration of "open word results"
---------------------------------------------------------------------------


Weak points
---------------------------------------------------------------------------
The authors give no details about classification methods. This makes it impossible for others to reproduce results, but also it gives no indication of how generalizable or robust their approach is.
Also, this makes it hard to understand why one approach performs better than the other or is more suited for other works.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #4
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                           Overall Value: -1

Summary of ideas
---------------------------------------------------------------------------
The paper describes an "attack" aimed at leaking web browsing activity of target users through the use of ML model trained on side channel data from Hardware Performance Counters (HPCs). While the model seems effective, the reviewers disputes the notion of this being an attack, as it is not clear how the side channel information can be gained. It is also not clear how machine-specific the model is.
---------------------------------------------------------------------------


Strong points
---------------------------------------------------------------------------
The experimental results seem to indicate a high level of efficacy in identifying the page visited by the user compared to existing results. The authors also mention no separate website is required to perform the attack, although this claim is disputable. While it is true users are not required to visit a specific website, it is not clear to this reviewer how the attack can be launched on the user computer, since the paper focuses on the ML fingerprinting model.
---------------------------------------------------------------------------


Weak points
---------------------------------------------------------------------------
Two main week points:
- the model seems to be highly specific to the machine over which it is being trained. The authors do not provide any experimental results on other hardware, raising the doubt that the model would only be successful in fingerprinting/classifying website on the exact same hardware and software configuration. This would require the attacker to train the model "online": either on the same machine, or with a data-feed from that machine. Both approaches significantly reduce the applicability of the attack. This point needs to be addressed before the paper can be considered for acceptance/publication.
- the authors provide little details on how the attacker can gain access to the HPC data. In the experimental set up the authors use perf: but even if perf was available on the target machine, by default access to the data would not be available to regular users (/proc/sys/kernel/perf_event_paranoid is normally set to 2, while the authors assume it is set to -1 in the paper). If the authors aim to define their contribution as an attack, they should be able to define how the attacker can gain access to such information on the user machine. This is largely missing from the paper, weakening significantly the contribution.

The paper would also need to be improved with regards to language.
---------------------------------------------------------------------------


Other comments
---------------------------------------------------------------------------
While the paper presents interesting results, it will require significant additional work to be ready for publication.
